When Na\"ive Bayes Nearest Neighbours Meet Convolutional Neural Networks

Since Convolutional Neural Networks (CNNs) have become the leading learning paradigm in visual recognition, Naive Bayes Nearest Neighbour (NBNN)-based classifiers have lost momentum in the community. This is because (1) such algorithms cannot use CNN activations as input features; (2) they cannot be used as final layer of CNN architectures for end-to-end training , and (3) they are generally not scalable and hence cannot handle big data. This paper proposes a framework that addresses all these issues, thus bringing back NBNNs on the map. We solve the first by extracting CNN activations from local patches at multiple scale levels, similarly to [1]. We address simultaneously the second and third by proposing a scalable version of Naive Bayes Non-linear Learning (NBNL, [2]). Results obtained using pre-trained CNNs on standard scene and domain adaptation databases show the strength of our approach, opening a new season for NBNNs.

==> da_tables.tex <==
\begin{table}[]
\centering
\caption{Unsupervised adaptation results on Office+Caltech 10}
\label{table:unsupervised-da}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Method \textbackslash Dataset & A-\textgreater W & A-\textgreater C & W-\textgreater A & W-\textgreater C & C-\textgreater A & C-\textgreater W \\
\hline
NBNN (Surf)                   & $31.8 $           & $31.3$            & $37.4 $           & $26.8$            & $41   $           & $28.4 $           \\
DA-NBNN (Surf)                & $35   $           & $41  $            & $42   $           & $33  $            & $55   $           & $36   $           \\
NBNN (CNN)                    & $60.23$           & $75.2$            & $66.87$           & $63.3$            & $79.03$           & $61.28$           \\
\hline
SGF                           &  $55.76$ & & & & & \\  
GFK \\
LapCNN\cite{long2015learning}                        &                 & $83.6$            &                 & $77.8$            & $92.1$            & $81.6$            \\
DDC\cite{long2015learning}                           &                 & $84.3$            &                 & $76.9$            & $91.3$            & $85.5$            \\
DAN\cite{long2015learning}                           &                 & $86  $            &                 & $81.5$            & $92  $            &                 \\
\hline
\end{tabular}
}
\end{table}
%
\begin{table}[]
\centering
\caption{Semi supervised adaptation results on Office+Caltech 10}
\label{table:semisupervised-da}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Method \textbackslash Dataset & A-\textgreater W & A-\textgreater C & W-\textgreater A & W-\textgreater C & C-\textgreater A & C-\textgreater W \\
\hline
NBNN (Surf)                   & $56.9$            & $34$              & $43.5$            & $31.6$            & $50.2$            & $57.7$            \\
DA-NBNN (Surf)                & $62$              & $46$              & $58$              & $42$              & $65$              & $61$              \\
NBNN (CNN)                    & $\mathbf{88.9}$            & $\mathbf{76.93}$           & $\mathbf{80.6}$            & $\mathbf{70.5}$            & $\mathbf{84.65}$           & $\mathbf{89.75}$           \\
\hline
H-L2L(LP-$\beta$)\cite{patricia2014learning}& $77.1$ & $38.6$ & $51.6$ & $34.0$ & $55.32$ &  \\ 
DASH-N\cite{nguyen2013non}                        & $75.5$            & $54.9$            & $70.4$            & $50.2$            & $71.6$            &                 \\
SDDL\cite{shekhar2013generalized}                 & $72$             & $27.4$          & $49.4$            & $29.7$            & $49.5$            &                 \\
HMP\cite{bo2011hierarchical}                      & $70$              & $51.7$            & $61.5$            & $46.8$            & $67.7$            &                 \\
\hline
\end{tabular}
}
\end{table}
%
\begin{table}[]
\centering
\caption{Source only \ac{NBNN} - 32px and 64px patches}
\label{table:da_source}
\resizebox{0.5\textwidth}{!}{%
$\begin{array}{|l|c|c|c|c|}
\hline
\text{Source \textbackslash Target}        & \text{Amazon}         & \text{Webcam}         & \text{DSLR}           & \text{Caltech256}     \\
\hline
\text{Amazon } & 89.85 \pm 0.64 & 59.89 \pm 2.55 & 68.28 \pm 4.95 & 75.76 \pm 1.33 \\
\text{Webcam } & 66.53 \pm 1.33 & 98.48 \pm 1.29 & 98.21 \pm 0.98 & 62.53 \pm 1.25 \\
\text{DSLR   } & 67.27 \pm 1.14 & 94 \pm 0.57    & 97.18 \pm 1.77 & 65.35 \pm 0.66 \\
\text{Caltech} & 78.81 \pm 0.84 & 61.25 \pm 4.4  & 66.75 \pm 6.26 & 80.5 \pm 1.42  \\
\hline
\end{array}$
}
\end{table}
%
\begin{table}[]
\centering
\caption{Source only \ac{NBNL} - 32px and 64px patches ReLU}
\label{table:da_nbnl_source}
\resizebox{0.5\textwidth}{!}{%
$\begin{array}{|l|c|c|c|c|}
\hline
\text{Source \textbackslash Target}        & \text{Amazon}         & \text{Webcam}         & \text{DSLR}           & \text{Caltech256}     \\
\hline
\text{Amazon } & -              & 61.93 \pm 3.75 & 71.21 \pm 3.2  & 72 \pm 2 \\
\text{Webcam } & 63.45 \pm 1.9  & -              & 96.43 \pm 1.51 & 55.81 \pm 1.5 \\
\text{DSLR   } & 61.12 \pm 1.5  & 85.83 \pm 1.64 & -              & 55.06 \pm 1.08 \\
\text{Caltech} & 80.91 \pm 2.0  & 64.84 \pm 3.42 & 73.64 \pm 3.03 & -            \\
\hline
\end{array}$
}
\end{table}
%
% \begin{table}[]
% \centering
% \caption{Source only \ac{NBNL} - 32px and 64px patches}
% \label{table:da_nbnl_source}
% \resizebox{0.5\textwidth}{!}{%
% $\begin{array}{|l|c|c|c|c|}
% \hline
% \text{Source \textbackslash Target}        & \text{Amazon}         & \text{Webcam}         & \text{DSLR}           & \text{Caltech256}     \\
% \hline
% \text{Amazon } & -              & 62.47 \pm 3.13 &  66.11 \pm 3.86 & 72.85 \pm 2.58\\
% \text{Webcam } & 57.1 \pm 2.5   & -              & 95.03 \pm 2.6   & 51.8 \pm 1.72  \\
% \text{DSLR   } & 58.43 \pm 3.25 & 87.43 \pm 2.03 & -               & 53.82 \pm 1.62  \\
% \text{Caltech} & 79.34 \pm 2.6  & 62.84 \pm 2.69 & 70.7 \pm 3.62   & -    \\
% \hline
% \end{array}$
% }
% \end{table}

%
\begin{table}[]
\centering
\caption{Source + 3 target images \ac{NBNN} - using 32px and 64px patches}
\label{table:da_source_t}
\resizebox{0.5\textwidth}{!}{%
$\begin{array}{|l|c|c|c|c|}
\hline
\text{Source \textbackslash Target}        & \text{Amazon}         & \text{Webcam}         & \text{DSLR}           & \text{Caltech256}     \\
\hline
\text{Amazon } & 90.53 \pm 0.87 & 88.981 \pm 0.87 & 93.46 \pm 1.23 & 76.96 \pm 1.72 \\
\text{Webcam } & 80.11 \pm 1.75 & 98.696 \pm 1.75 & 99.21 \pm 0.83 & 69.89 \pm 1.64  \\
\text{DSLR   } & 81.34 \pm 1.88 & 97.057 \pm 1.88 & 97.94 \pm 1.98 & 72.86 \pm 0.93 \\
\text{Caltech} & 84.66 \pm 1.28 & 90.038 \pm 1.28 & 93.07 \pm 2.09 & 81.01 \pm 0.80  \\
\hline
\end{array}$
}
\end{table}
%
\begin{table}[]
\centering
\caption{Source + Target \ac{NBNL} - 32px and 64px patches ReLU}
\label{table:da_nbnl_source}
\resizebox{0.5\textwidth}{!}{%
$\begin{array}{|l|c|c|c|c|}
\hline
\text{Source \textbackslash Target}        & \text{Amazon}         & \text{Webcam}         & \text{DSLR}           & \text{Caltech256}     \\
\hline
\text{Amazon }  & -              & 87.54 \pm 2.35 & 90.47 \pm 3.23 & 76.74 \pm 1.9  \\
\text{Webcam }  & 79.38 \pm 1.64 & -              & 98.91 \pm 0.7  & 70.17 \pm 1.69 \\
\text{DSLR   }  & 81.16 \pm 1.63 & 94.94 \pm 1.44 & -              & 70.66 \pm 1.7  \\
\text{Caltech}  & 85.62 \pm 1.14 & 87.28 \pm 2.52 & 90.55 \pm 1.99 & -              \\
\hline
\end{array}$
}
\end{table}

Amazon  & -              & 87.54 \pm 2.35 & 90.47 \pm 3.23 & 76.74 \pm 1.9  \\
Webcam  & 79.38 \pm 1.64 & -              & 98.91 \pm 0.7  & 70.17 \pm 1.69 \\
DSLR    & 81.16 \pm 1.63 & 94.94 \pm 1.44 & -              & 70.66 \pm 1.7  \\
Caltech & 85.62 \pm 1.14 & 87.28 \pm 2.52 & 90.55 \pm 1.99 & -             

==> tables.tex <==
% \begin{table}[]
% \centering
% \caption{$p-value$ of the two-sided sign test between showcased methods}
% \label{table:sign-test}
% \begin{tabular}{|l|ccc|}
% \hline
% Method \textbackslash Dataset     & Scenes 15 & Sports 8 & ISR 67 \\
% \hline
% \small{\ac{NBNL} / \ac{STOML3} (CNN)}  & $0.375$     & $1$        & $1$      \\
% NBNL - NBNN                       & $0.06$     & $0.06$     & $0.06$   \\
% \hline
% \end{tabular}
% \end{table}

\begin{table}[]
\centering
\caption{Comparison results between the best features on scene classification. courtesy of \cite{zuo2015exemplar}}
\label{table:feature-comparison}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
Methods                         & Scene $15$ & Sports$8$ & MIT$67$  \\
\hline
SIFT                   		& $82.06$         & $85.12$            & $45.86$           \\
OTC                   		& $84.37$         & $-$                   & $47.33$           \\
DDSFL                           & $84.42$         & $86.91$            & $52.26$           \\
Caffe-Imagenet     		& $87.99$         & $93.96$            & $58.52$           \\
Caffe-Hybrid		        & $91.59$         & $94.22$            & $70.80$           \\
SIFT + Caffe                    & $89.90$         & $95.05$            & $70.51$           \\
DDSFL + Caffe                   & $92.81$         & $96.78$            & $76.23$          \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[]
\centering
\caption{Comparison of best methods on Scenes with ours - \textbf{bold} is best of single feature method, \textcolor{red}{\textbf{red bold}} is overall best }
\label{table:method-comparison}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
Method        & Scene $15$ & Sports $8$ & MIT$67$ \\
\hline
NBNN (Surf)\cite{fornoni2014scene}   & $72.8$     & $67.6$     & $-$      \\
NBNL (Surf)\cite{fornoni2014scene}   & $82.42$    & $85.54$    & $42.15$ \\
NBNN (CNN)    & $88.24 \pm 0.99$    & $94.46 \pm 0.47$    & $63.92 \pm 1.63$ \\
Lin. SVM(CNN) & $90 \pm 0.63$   & $94.16 \pm 1.13$ & $64.62 \pm 1.04$ \\
NBNL (CNN)    & $92.42 \pm 0.64$    & $\mathbf{95.29 \pm 0.61}$    & $\mathbf{73 \pm 0.36}$    \\
\small{\ac{NBNL} / \ac{STOML3} (CNN)}    & \textcolor{red}{$\mathbf{92.88 \pm 0.89}$}    & $95.28 \pm 0.68$    & $72.63 \pm 0.45$    \\
\hline
Hybrid CNN\cite{zhou2014learning}    & $91.59$    & $94.22$    & $70.8$  \\
LScSPM\cite{gao2013laplacian}        & $89.78$    & $85.27$    & $-$    \\
MOP-CNN\cite{gong2014multi}          &  $-$       &  $-$        & $68.88$ \\
\hline
DDSFL + CAFFE\cite{zuo2015exemplar} & $92.81$    & \textcolor{red}{$\mathbf{96.78}$}    & \textcolor{red}{$\mathbf{76.23}$} \\
ISPR + IFV\cite{lin2014learning}    & $91.06$    & $92.08$    & $68.50$ \\
CNN Fusion\cite{koskela2014convolutional} & $92.1$ & $94.8$ & $70.1$ \\
\hline
\end{tabular}
}
\end{table}

\begin{table}[]
\centering
\caption{NBNL - STOML3 comparison, 64px and 128px ReLU}
\label{table:nbnl_snbnl_comparison}
\resizebox{0.5\textwidth}{!}{%
$\begin{array}{|l|c|c|c|c|c|c|c|c|c|}
\hline
               & \multicolumn{3}{|c|}{\text{\text{Sports 8}}} & \multicolumn{3}{|c|}{\text{Scenes 15}} & \multicolumn{3}{|c|}{\text{ISR 67}}  \\
\hline
               & \text{Acc.}    & \text{Train T.} & \text{Test T.} & \text{Acc}     & \text{Train T.}  & \text{Test T.} & \text{Acc.}   & \text{Train T.} & \text{Test T.} \\
\hline
\text{NBNL}     & 94.29   & 1024.4   & 13.9    & 91.5    & 5729.2    & 95.9    & 72.592 & 9690     & 63.2    \\
\text{SNBNL}    & 95.268  & 63.564   & 0.404   & 91.638  & 210.3     & 1.9     & 72.786 & 304.26   & 1.3     \\
\hline
\text{Speed Up} & -      & 16x       & 34x      &    -     & 27x        & 50x      &   -     & 32x       & 49x      \\
\hline
\end{array}$
}
\end{table}

